Importance-based Neuron Allocation for Multilingual Neural Machine Translation

Multilingual neural machine translation with a single model has drawn much attention due to its capability to deal with multiple languages. However, the current multilingual translation paradigm often makes the model tend to preserve the general knowledge, but ignore the language-specific knowledge. Some previous works try to solve this problem by adding various kinds of language-specific modules to the model, but they suffer from the parameter explosion problem and require specialized manual design. To solve these problems, we propose to divide the model neurons into general and language-specific parts based on their importance across languages. The general part is responsible for preserving the general knowledge and participating in the translation of all the languages, while the language-specific part is responsible for preserving the language-specific knowledge and participating in the translation of some specific languages. Experimental results on several language pairs, covering IWSLT and Europarl corpus datasets, demonstrate the effectiveness and universality of the proposed method.

==> temp <==
@inproceedings{DBLP:conf/nips/RaghuGYS17,
  author    = {Maithra Raghu and
               Justin Gilmer and
               Jason Yosinski and
               Jascha Sohl{-}Dickstein},
  title     = {{SVCCA:} Singular Vector Canonical Correlation Analysis for Deep Learning
               Dynamics and Interpretability},
  booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
               on Neural Information Processing Systems 2017, 4-9 December 2017,
               Long Beach, CA, {USA}},
  pages     = {6076--6085},
  year      = {2017},
  crossref  = {DBLP:conf/nips/2017},
  url       = {http://papers.nips.cc/paper/7188-svcca-singular-vector-canonical-correlation-analysis-for-deep-learning-dynamics-and-interpretability},
  timestamp = {Fri, 06 Mar 2020 17:00:40 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/RaghuGYS17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/emnlp/KalchbrennerB13,
  author    = {Nal Kalchbrenner and
               Phil Blunsom},
  title     = {Recurrent Continuous Translation Models},
  booktitle = {Proceedings of the 2013 Conference on Empirical Methods in Natural
               Language Processing, {EMNLP} 2013, 18-21 October 2013, Grand Hyatt
               Seattle, Seattle, Washington, USA, {A} meeting of SIGDAT, a Special
               Interest Group of the {ACL}},
  pages     = {1700--1709},
  year      = {2013},
  crossref  = {DBLP:conf/emnlp/2013},
  url       = {https://www.aclweb.org/anthology/D13-1176/},
  timestamp = {Fri, 13 Sep 2019 13:08:45 +0200},
  biburl    = {https://dblp.org/rec/conf/emnlp/KalchbrennerB13.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/nips/SutskeverVL14,
  author    = {Ilya Sutskever and
               Oriol Vinyals and
               Quoc V. Le},
  title     = {Sequence to Sequence Learning with Neural Networks},
  booktitle = {Advances in Neural Information Processing Systems 27: Annual Conference
               on Neural Information Processing Systems 2014, December 8-13 2014,
               Montreal, Quebec, Canada},
  pages     = {3104--3112},
  year      = {2014},
  crossref  = {DBLP:conf/nips/2014},
  url       = {http://papers.nips.cc/paper/5346-sequence-to-sequence-learning-with-neural-networks},
  timestamp = {Fri, 06 Mar 2020 16:58:11 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/SutskeverVL14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:journals/corr/BahdanauCB14,
  author    = {Dzmitry Bahdanau and
               Kyunghyun Cho and
               Yoshua Bengio},
  title     = {Neural Machine Translation by Jointly Learning to Align and Translate},
  booktitle = {3rd International Conference on Learning Representations, {ICLR} 2015,
               San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings},
  year      = {2015},
  crossref  = {DBLP:conf/iclr/2015},
  url       = {http://arxiv.org/abs/1409.0473},
  timestamp = {Wed, 17 Jul 2019 10:40:54 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/BahdanauCB14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icml/GehringAGYD17,
  author    = {Jonas Gehring and
               Michael Auli and
               David Grangier and
               Denis Yarats and
               Yann N. Dauphin},
  title     = {Convolutional Sequence to Sequence Learning},
  booktitle = {Proceedings of the 34th International Conference on Machine Learning,
               {ICML} 2017, Sydney, NSW, Australia, 6-11 August 2017},
  pages     = {1243--1252},
  year      = {2017},
  crossref  = {DBLP:conf/icml/2017},
  url       = {http://proceedings.mlr.press/v70/gehring17a.html},
  timestamp = {Wed, 29 May 2019 08:41:45 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/GehringAGYD17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/nips/VaswaniSPUJGKP17,
  author    = {Ashish Vaswani and
               Noam Shazeer and
               Niki Parmar and
               Jakob Uszkoreit and
               Llion Jones and
               Aidan N. Gomez and
               Lukasz Kaiser and
               Illia Polosukhin},
  title     = {Attention is All you Need},
  booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
               on Neural Information Processing Systems 2017, 4-9 December 2017,
               Long Beach, CA, {USA}},
  pages     = {5998--6008},
  year      = {2017},
  crossref  = {DBLP:conf/nips/2017},
  url       = {http://papers.nips.cc/paper/7181-attention-is-all-you-need},
  timestamp = {Fri, 06 Mar 2020 17:00:11 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/VaswaniSPUJGKP17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/emnlp/TanCHXQL19,
  author    = {Xu Tan and
               Jiale Chen and
               Di He and
               Yingce Xia and
               Tao Qin and
               Tie{-}Yan Liu},
  title     = {Multilingual Neural Machine Translation with Language Clustering},
  booktitle = {Proceedings of the 2019 Conference on Empirical Methods in Natural
               Language Processing and the 9th International Joint Conference on
               Natural Language Processing, {EMNLP-IJCNLP} 2019, Hong Kong, China,
               November 3-7, 2019},
  pages     = {963--973},
  year      = {2019},
  crossref  = {DBLP:conf/emnlp/2019-1},
  url       = {https://doi.org/10.18653/v1/D19-1089},
  doi       = {10.18653/v1/D19-1089},
  timestamp = {Thu, 12 Dec 2019 13:23:45 +0100},
  biburl    = {https://dblp.org/rec/conf/emnlp/TanCHXQL19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/tacl/JohnsonSLKWCTVW17,
  author    = {Melvin Johnson and
               Mike Schuster and
               Quoc V. Le and
               Maxim Krikun and
               Yonghui Wu and
               Zhifeng Chen and
               Nikhil Thorat and
               Fernanda B. Vi{\'{e}}gas and
               Martin Wattenberg and
               Greg Corrado and
               Macduff Hughes and
               Jeffrey Dean},
  title     = {Google's Multilingual Neural Machine Translation System: Enabling
               Zero-Shot Translation},
  journal   = {{TACL}},
  volume    = {5},
  pages     = {339--351},
  year      = {2017},
  url       = {https://transacl.org/ojs/index.php/tacl/article/view/1081},
  timestamp = {Fri, 03 Nov 2017 17:02:32 +0100},
  biburl    = {https://dblp.org/rec/journals/tacl/JohnsonSLKWCTVW17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/HaNW16,
  author    = {Thanh{-}Le Ha and
               Jan Niehues and
               Alexander H. Waibel},
  title     = {Toward Multilingual Neural Machine Translation with Universal Encoder
               and Decoder},
  journal   = {CoRR},
  volume    = {abs/1611.04798},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.04798},
  archivePrefix = {arXiv},
  eprint    = {1611.04798},
  timestamp = {Mon, 13 Aug 2018 16:46:26 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/HaNW16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/naacl/FiratCB16,
  author    = {Orhan Firat and
               Kyunghyun Cho and
               Yoshua Bengio},
  title     = {Multi-Way, Multilingual Neural Machine Translation with a Shared Attention
               Mechanism},
  booktitle = {{NAACL} {HLT} 2016, The 2016 Conference of the North American Chapter
               of the Association for Computational Linguistics: Human Language Technologies,
               San Diego California, USA, June 12-17, 2016},
  pages     = {866--875},
  year      = {2016},
  crossref  = {DBLP:conf/naacl/2016},
  url       = {https://doi.org/10.18653/v1/n16-1101},
  doi       = {10.18653/v1/n16-1101},
  timestamp = {Tue, 28 Jan 2020 10:30:10 +0100},
  biburl    = {https://dblp.org/rec/conf/naacl/FiratCB16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/wmt/LuKLBZS18,
  author    = {Yichao Lu and
               Phillip Keung and
               Faisal Ladhak and
               Vikas Bhardwaj and
               Shaonan Zhang and
               Jason Sun},
  title     = {A neural interlingua for multilingual machine translation},
  booktitle = {Proceedings of the Third Conference on Machine Translation: Research
               Papers, {WMT} 2018, Belgium, Brussels, October 31 - November 1, 2018},
  pages     = {84--92},
  year      = {2018},
  crossref  = {DBLP:conf/wmt/2018},
  url       = {https://doi.org/10.18653/v1/w18-6309},
  doi       = {10.18653/v1/w18-6309},
  timestamp = {Tue, 28 Jan 2020 10:31:03 +0100},
  biburl    = {https://dblp.org/rec/conf/wmt/LuKLBZS18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/acl/WangZZZXZ19,
  author    = {Yining Wang and
               Long Zhou and
               Jiajun Zhang and
               Feifei Zhai and
               Jingfang Xu and
               Chengqing Zong},
  title     = {A Compact and Language-Sensitive Multilingual Translation Method},
  booktitle = {Proceedings of the 57th Conference of the Association for Computational
               Linguistics, {ACL} 2019, Florence, Italy, July 28- August 2, 2019,
               Volume 1: Long Papers},
  pages     = {1213--1223},
  year      = {2019},
  crossref  = {DBLP:conf/acl/2019-1},
  url       = {https://doi.org/10.18653/v1/p19-1117},
  doi       = {10.18653/v1/p19-1117},
  timestamp = {Tue, 28 Jan 2020 10:27:12 +0100},
  biburl    = {https://dblp.org/rec/conf/acl/WangZZZXZ19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/naacl/GuHDL18,
  author    = {Jiatao Gu and
               Hany Hassan and
               Jacob Devlin and
               Victor O. K. Li},
  title     = {Universal Neural Machine Translation for Extremely Low Resource Languages},
  booktitle = {Proceedings of the 2018 Conference of the North American Chapter of
               the Association for Computational Linguistics: Human Language Technologies,
               {NAACL-HLT} 2018, New Orleans, Louisiana, USA, June 1-6, 2018, Volume
               1 (Long Papers)},
  pages     = {344--354},
  year      = {2018},
  crossref  = {DBLP:conf/naacl/2018-1},
  url       = {https://doi.org/10.18653/v1/n18-1032},
  doi       = {10.18653/v1/n18-1032},
  timestamp = {Tue, 28 Jan 2020 10:30:28 +0100},
  biburl    = {https://dblp.org/rec/conf/naacl/GuHDL18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/ijcai/XiaoLZ0L19,
  author    = {Tong Xiao and
               Yinqiao Li and
               Jingbo Zhu and
               Zhengtao Yu and
               Tongran Liu},
  title     = {Sharing Attention Weights for Fast Transformer},
  booktitle = {Proceedings of the Twenty-Eighth International Joint Conference on
               Artificial Intelligence, {IJCAI} 2019, Macao, China, August 10-16,
               2019},
  pages     = {5292--5298},
  year      = {2019},
  crossref  = {DBLP:conf/ijcai/2019},
  url       = {https://doi.org/10.24963/ijcai.2019/735},
  doi       = {10.24963/ijcai.2019/735},
  timestamp = {Tue, 20 Aug 2019 16:18:18 +0200},
  biburl    = {https://dblp.org/rec/conf/ijcai/XiaoLZ0L19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/acl/WangLXZLWC19,
  author    = {Qiang Wang and
               Bei Li and
               Tong Xiao and
               Jingbo Zhu and
               Changliang Li and
               Derek F. Wong and
               Lidia S. Chao},
  title     = {Learning Deep Transformer Models for Machine Translation},
  booktitle = {Proceedings of the 57th Conference of the Association for Computational
               Linguistics, {ACL} 2019, Florence, Italy, July 28- August 2, 2019,
               Volume 1: Long Papers},
  pages     = {1810--1822},
  year      = {2019},
  crossref  = {DBLP:conf/acl/2019-1},
  url       = {https://doi.org/10.18653/v1/p19-1176},
  doi       = {10.18653/v1/p19-1176},
  timestamp = {Tue, 28 Jan 2020 10:27:53 +0100},
  biburl    = {https://dblp.org/rec/conf/acl/WangLXZLWC19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icml/BengioLCW09,
  author    = {Yoshua Bengio and
               J{\'{e}}r{\^{o}}me Louradour and
               Ronan Collobert and
               Jason Weston},
  title     = {Curriculum learning},
  booktitle = {Proceedings of the 26th Annual International Conference on Machine
               Learning, {ICML} 2009, Montreal, Quebec, Canada, June 14-18, 2009},
  pages     = {41--48},
  year      = {2009},
  crossref  = {DBLP:conf/icml/2009},
  url       = {https://doi.org/10.1145/1553374.1553380},
  doi       = {10.1145/1553374.1553380},
  timestamp = {Wed, 14 Nov 2018 10:58:56 +0100},
  biburl    = {https://dblp.org/rec/conf/icml/BengioLCW09.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{elman1993learning,
  title={Learning and development in neural networks: The importance of starting small},
  author={Elman, Jeffrey L},
  journal={Cognition},
  volume={48},
  number={1},
  pages={71--99},
  year={1993},
  publisher={Elsevier}
}

@inproceedings{DBLP:conf/icml/WeinshallCA18,
  author    = {Daphna Weinshall and
               Gad Cohen and
               Dan Amir},
  title     = {Curriculum Learning by Transfer Learning: Theory and Experiments with
               Deep Networks},
  booktitle = {Proceedings of the 35th International Conference on Machine Learning,
               {ICML} 2018, Stockholmsm{\"{a}}ssan, Stockholm, Sweden, July
               10-15, 2018},
  pages     = {5235--5243},
  year      = {2018},
  crossref  = {DBLP:conf/icml/2018},
  url       = {http://proceedings.mlr.press/v80/weinshall18a.html},
  timestamp = {Wed, 03 Apr 2019 18:17:30 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/WeinshallCA18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/eacl/FaruquiD14,
  author    = {Manaal Faruqui and
               Chris Dyer},
  title     = {Improving Vector Space Word Representations Using Multilingual Correlation},
  booktitle = {Proceedings of the 14th Conference of the European Chapter of the
               Association for Computational Linguistics, {EACL} 2014, April 26-30,
               2014, Gothenburg, Sweden},
  pages     = {462--471},
  year      = {2014},
  crossref  = {DBLP:conf/eacl/2014},
  url       = {https://doi.org/10.3115/v1/e14-1049},
  doi       = {10.3115/v1/e14-1049},
  timestamp = {Tue, 28 Jan 2020 10:31:09 +0100},
  biburl    = {https://dblp.org/rec/conf/eacl/FaruquiD14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/emnlp/KuduguntaBCF19,
  author    = {Sneha Reddy Kudugunta and
               Ankur Bapna and
               Isaac Caswell and
               Orhan Firat},
  title     = {Investigating Multilingual {NMT} Representations at Scale},
  booktitle = {Proceedings of the 2019 Conference on Empirical Methods in Natural
               Language Processing and the 9th International Joint Conference on
               Natural Language Processing, {EMNLP-IJCNLP} 2019, Hong Kong, China,
               November 3-7, 2019},
  pages     = {1565--1575},
  year      = {2019},
  crossref  = {DBLP:conf/emnlp/2019-1},
  url       = {https://doi.org/10.18653/v1/D19-1167},
  doi       = {10.18653/v1/D19-1167},
  timestamp = {Thu, 12 Dec 2019 13:23:46 +0100},
  biburl    = {https://dblp.org/rec/conf/emnlp/KuduguntaBCF19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/naacl/PlataniosSNPM19,
  author    = {Emmanouil Antonios Platanios and
               Otilia Stretcu and
               Graham Neubig and
               Barnab{\'{a}}s P{\'{o}}czos and
               Tom M. Mitchell},
  title     = {Competence-based Curriculum Learning for Neural Machine Translation},
  booktitle = {Proceedings of the 2019 Conference of the North American Chapter of
               the Association for Computational Linguistics: Human Language Technologies,
               {NAACL-HLT} 2019, Minneapolis, MN, USA, June 2-7, 2019, Volume 1 (Long
               and Short Papers)},
  pages     = {1162--1172},
  year      = {2019},
  crossref  = {DBLP:conf/naacl/2019-1},
  url       = {https://doi.org/10.18653/v1/n19-1119},
  doi       = {10.18653/v1/n19-1119},
  timestamp = {Tue, 28 Jan 2020 10:30:17 +0100},
  biburl    = {https://dblp.org/rec/conf/naacl/PlataniosSNPM19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/naacl/ZhangSKMCD19,
  author    = {Xuan Zhang and
               Pamela Shapiro and
               Gaurav Kumar and
               Paul McNamee and
               Marine Carpuat and
               Kevin Duh},
  title     = {Curriculum Learning for Domain Adaptation in Neural Machine Translation},
  booktitle = {Proceedings of the 2019 Conference of the North American Chapter of
               the Association for Computational Linguistics: Human Language Technologies,
               {NAACL-HLT} 2019, Minneapolis, MN, USA, June 2-7, 2019, Volume 1 (Long
               and Short Papers)},
  pages     = {1903--1915},
  year      = {2019},
  crossref  = {DBLP:conf/naacl/2019-1},
  url       = {https://doi.org/10.18653/v1/n19-1189},
  doi       = {10.18653/v1/n19-1189},
  timestamp = {Tue, 28 Jan 2020 10:30:24 +0100},
  biburl    = {https://dblp.org/rec/conf/naacl/ZhangSKMCD19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-1811-00739,
  author    = {Xuan Zhang and
               Gaurav Kumar and
               Huda Khayrallah and
               Kenton Murray and
               Jeremy Gwinnup and
               Marianna J. Martindale and
               Paul McNamee and
               Kevin Duh and
               Marine Carpuat},
  title     = {An Empirical Exploration of Curriculum Learning for Neural Machine
               Translation},
  journal   = {CoRR},
  volume    = {abs/1811.00739},
  year      = {2018},
  url       = {http://arxiv.org/abs/1811.00739},
  archivePrefix = {arXiv},
  eprint    = {1811.00739},
  timestamp = {Thu, 22 Nov 2018 17:58:30 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1811-00739.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/ranlp/KocmiB17,
  author    = {Tom Kocmi and
               Ondrej Bojar},
  title     = {Curriculum Learning and Minibatch Bucketing in Neural Machine Translation},
  booktitle = {Proceedings of the International Conference Recent Advances in Natural
               Language Processing, {RANLP} 2017, Varna, Bulgaria, September 2 -
               8, 2017},
  pages     = {379--386},
  year      = {2017},
  crossref  = {DBLP:conf/ranlp/2017},
  url       = {https://doi.org/10.26615/978-954-452-049-6\_050},
  doi       = {10.26615/978-954-452-049-6\_050},
  timestamp = {Wed, 18 Sep 2019 12:47:55 +0200},
  biburl    = {https://dblp.org/rec/conf/ranlp/KocmiB17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/naacl/KumarFCK19,
  author    = {Gaurav Kumar and
               George Foster and
               Colin Cherry and
               Maxim Krikun},
  title     = {Reinforcement Learning based Curriculum Optimization for Neural Machine
               Translation},
  booktitle = {Proceedings of the 2019 Conference of the North American Chapter of
               the Association for Computational Linguistics: Human Language Technologies,
               {NAACL-HLT} 2019, Minneapolis, MN, USA, June 2-7, 2019, Volume 1 (Long
               and Short Papers)},
  pages     = {2054--2061},
  year      = {2019},
  crossref  = {DBLP:conf/naacl/2019-1},
  url       = {https://doi.org/10.18653/v1/n19-1208},
  doi       = {10.18653/v1/n19-1208},
  timestamp = {Tue, 28 Jan 2020 10:30:16 +0100},
  biburl    = {https://dblp.org/rec/conf/naacl/KumarFCK19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/wmt/WangWHNC18,
  author    = {Wei Wang and
               Taro Watanabe and
               Macduff Hughes and
               Tetsuji Nakagawa and
               Ciprian Chelba},
  title     = {Denoising Neural Machine Translation Training with Trusted Data and
               Online Data Selection},
  booktitle = {Proceedings of the Third Conference on Machine Translation: Research
               Papers, {WMT} 2018, Belgium, Brussels, October 31 - November 1, 2018},
  pages     = {133--143},
  year      = {2018},
  crossref  = {DBLP:conf/wmt/2018},
  url       = {https://doi.org/10.18653/v1/w18-6314},
  doi       = {10.18653/v1/w18-6314},
  timestamp = {Tue, 28 Jan 2020 10:30:58 +0100},
  biburl    = {https://dblp.org/rec/conf/wmt/WangWHNC18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{DBLP:conf/aaai/ZhaoWNW20,
  author    = {Mingjun Zhao and
               Haijiang Wu and
               Di Niu and
               Xiaoli Wang},
  title     = {Reinforced Curriculum Learning on Pre-Trained Neural Machine Translation
               Models},
  booktitle = {The Thirty-Fourth {AAAI} Conference on Artificial Intelligence, {AAAI}
               2020, The Thirty-Second Innovative Applications of Artificial Intelligence
               Conference, {IAAI} 2020, The Tenth {AAAI} Symposium on Educational
               Advances in Artificial Intelligence, {EAAI} 2020, New York, NY, USA,
               February 7-12, 2020},
  pages     = {9652--9659},
  publisher = {{AAAI} Press},
  year      = {2020},
  url       = {https://aaai.org/ojs/index.php/AAAI/article/view/6513},
  timestamp = {Thu, 04 Jun 2020 13:18:48 +0200},
  biburl    = {https://dblp.org/rec/conf/aaai/ZhaoWNW20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-1911-08717,
  author    = {Junliang Guo and
               Xu Tan and
               Linli Xu and
               Tao Qin and
               Enhong Chen and
               Tie{-}Yan Liu},
  title     = {Fine-Tuning by Curriculum Learning for Non-Autoregressive Neural Machine
               Translation},
  journal   = {CoRR},
  volume    = {abs/1911.08717},
  year      = {2019},
  url       = {http://arxiv.org/abs/1911.08717},
  archivePrefix = {arXiv},
  eprint    = {1911.08717},
  timestamp = {Tue, 03 Dec 2019 14:15:54 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1911-08717.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/acl/DongWHYW15,
  author    = {Daxiang Dong and
               Hua Wu and
               Wei He and
               Dianhai Yu and
               Haifeng Wang},
  title     = {Multi-Task Learning for Multiple Language Translation},
  booktitle = {Proceedings of the 53rd Annual Meeting of the Association for Computational
               Linguistics and the 7th International Joint Conference on Natural
               Language Processing of the Asian Federation of Natural Language Processing,
               {ACL} 2015, July 26-31, 2015, Beijing, China, Volume 1: Long Papers},
  pages     = {1723--1732},
  year      = {2015},
  crossref  = {DBLP:conf/acl/2015-1},
  url       = {https://doi.org/10.3115/v1/p15-1166},
  doi       = {10.3115/v1/p15-1166},
  timestamp = {Tue, 28 Jan 2020 10:27:57 +0100},
  biburl    = {https://dblp.org/rec/conf/acl/DongWHYW15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/emnlp/PlataniosSNM18,
  author    = {Emmanouil Antonios Platanios and
               Mrinmaya Sachan and
               Graham Neubig and
               Tom M. Mitchell},
  title     = {Contextual Parameter Generation for Universal Neural Machine Translation},
  booktitle = {Proceedings of the 2018 Conference on Empirical Methods in Natural
               Language Processing, Brussels, Belgium, October 31 - November 4, 2018},
  pages     = {425--435},
  year      = {2018},
  crossref  = {DBLP:conf/emnlp/2018},
  url       = {https://doi.org/10.18653/v1/d18-1039},
  doi       = {10.18653/v1/d18-1039},
  timestamp = {Tue, 28 Jan 2020 10:28:44 +0100},
  biburl    = {https://dblp.org/rec/conf/emnlp/PlataniosSNM18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:journals/corr/LuongLSVK15,
  author    = {Minh{-}Thang Luong and
               Quoc V. Le and
               Ilya Sutskever and
               Oriol Vinyals and
               Lukasz Kaiser},
  title     = {Multi-task Sequence to Sequence Learning},
  booktitle = {4th International Conference on Learning Representations, {ICLR} 2016,
               San Juan, Puerto Rico, May 2-4, 2016, Conference Track Proceedings},
  year      = {2016},
  crossref  = {DBLP:conf/iclr/2016},
  url       = {http://arxiv.org/abs/1511.06114},
  timestamp = {Thu, 25 Jul 2019 14:25:37 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/LuongLSVK15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/acl/SennrichHB16a,
  author    = {Rico Sennrich and
               Barry Haddow and
               Alexandra Birch},
  title     = {Neural Machine Translation of Rare Words with Subword Units},
  booktitle = {Proceedings of the 54th Annual Meeting of the Association for Computational
               Linguistics, {ACL} 2016, August 7-12, 2016, Berlin, Germany, Volume
               1: Long Papers},
  year      = {2016},
  crossref  = {DBLP:conf/acl/2016-1},
  url       = {https://doi.org/10.18653/v1/p16-1162},
  doi       = {10.18653/v1/p16-1162},
  timestamp = {Tue, 28 Jan 2020 10:28:06 +0100},
  biburl    = {https://dblp.org/rec/conf/acl/SennrichHB16a.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{ott2019fairseq,
  title = {fairseq: A Fast, Extensible Toolkit for Sequence Modeling},
  author = {Myle Ott and Sergey Edunov and Alexei Baevski and Angela Fan and Sam Gross and Nathan Ng and David Grangier and Michael Auli},
  booktitle = {Proceedings of NAACL-HLT 2019: Demonstrations},
  year = {2019},
}

@inproceedings{DBLP:journals/corr/KingmaB14,
  author    = {Diederik P. Kingma and
               Jimmy Ba},
  title     = {Adam: {A} Method for Stochastic Optimization},
  booktitle = {3rd International Conference on Learning Representations, {ICLR} 2015,
               San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings},
  year      = {2015},
  crossref  = {DBLP:conf/iclr/2015},
  url       = {http://arxiv.org/abs/1412.6980},
  timestamp = {Thu, 25 Jul 2019 14:25:37 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/KingmaB14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/acl/PapineniRWZ02,
  author    = {Kishore Papineni and
               Salim Roukos and
               Todd Ward and
               Wei{-}Jing Zhu},
  title     = {Bleu: a Method for Automatic Evaluation of Machine Translation},
  booktitle = {Proceedings of the 40th Annual Meeting of the Association for Computational
               Linguistics, July 6-12, 2002, Philadelphia, PA, {USA}},
  pages     = {311--318},
  year      = {2002},
  crossref  = {DBLP:conf/acl/2002},
  url       = {https://www.aclweb.org/anthology/P02-1040/},
  timestamp = {Tue, 17 Sep 2019 13:40:53 +0200},
  biburl    = {https://dblp.org/rec/conf/acl/PapineniRWZ02.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/interspeech/Stolcke02,
  author    = {Andreas Stolcke},
  title     = {{SRILM} - an extensible language modeling toolkit},
  booktitle = {7th International Conference on Spoken Language Processing, {ICSLP2002}
               - {INTERSPEECH} 2002, Denver, Colorado, USA, September 16-20, 2002},
  year      = {2002},
  crossref  = {DBLP:conf/interspeech/2002},
  url       = {http://www.isca-speech.org/archive/icslp\_2002/i02\_0901.html},
  timestamp = {Mon, 21 Mar 2011 15:38:48 +0100},
  biburl    = {https://dblp.org/rec/conf/interspeech/Stolcke02.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/naacl/DevlinCLT19,
  author    = {Jacob Devlin and
               Ming{-}Wei Chang and
               Kenton Lee and
               Kristina Toutanova},
  title     = {{BERT:} Pre-training of Deep Bidirectional Transformers for Language
               Understanding},
  booktitle = {Proceedings of the 2019 Conference of the North American Chapter of
               the Association for Computational Linguistics: Human Language Technologies,
               {NAACL-HLT} 2019, Minneapolis, MN, USA, June 2-7, 2019, Volume 1 (Long
               and Short Papers)},
  pages     = {4171--4186},
  year      = {2019},
  crossref  = {DBLP:conf/naacl/2019-1},
  url       = {https://doi.org/10.18653/v1/n19-1423},
  doi       = {10.18653/v1/n19-1423},
  timestamp = {Tue, 28 Jan 2020 10:30:29 +0100},
  biburl    = {https://dblp.org/rec/conf/naacl/DevlinCLT19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@misc{xiao2018bertservice,
  title={bert-as-service},
  author={Xiao, Han},
  howpublished={\url{https://github.com/hanxiao/bert-as-service}},
  year={2018}
}

@article{DBLP:journals/neco/HardoonSS04,
  author    = {David R. Hardoon and
               S{\'{a}}ndor Szedm{\'{a}}k and
               John Shawe{-}Taylor},
  title     = {Canonical Correlation Analysis: An Overview with Application to Learning
               Methods},
  journal   = {Neural Computation},
  volume    = {16},
  number    = {12},
  pages     = {2639--2664},
  year      = {2004},
  url       = {https://doi.org/10.1162/0899766042321814},
  doi       = {10.1162/0899766042321814},
  timestamp = {Wed, 25 Sep 2019 17:52:26 +0200},
  biburl    = {https://dblp.org/rec/journals/neco/HardoonSS04.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-1907-05019,
  author    = {Naveen Arivazhagan and
               Ankur Bapna and
               Orhan Firat and
               Dmitry Lepikhin and
               Melvin Johnson and
               Maxim Krikun and
               Mia Xu Chen and
               Yuan Cao and
               George F. Foster and
               Colin Cherry and
               Wolfgang Macherey and
               Zhifeng Chen and
               Yonghui Wu},
  title     = {Massively Multilingual Neural Machine Translation in the Wild: Findings
               and Challenges},
  journal   = {CoRR},
  volume    = {abs/1907.05019},
  year      = {2019},
  url       = {http://arxiv.org/abs/1907.05019},
  archivePrefix = {arXiv},
  eprint    = {1907.05019},
  timestamp = {Fri, 20 Mar 2020 09:13:26 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1907-05019.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/LHostisGA16,
  author    = {Gurvan L'Hostis and
               David Grangier and
               Michael Auli},
  title     = {Vocabulary Selection Strategies for Neural Machine Translation},
  journal   = {CoRR},
  volume    = {abs/1610.00072},
  year      = {2016},
  url       = {http://arxiv.org/abs/1610.00072},
  archivePrefix = {arXiv},
  eprint    = {1610.00072},
  timestamp = {Mon, 13 Aug 2018 16:46:42 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/LHostisGA16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/HintonVD15,
  author    = {Geoffrey E. Hinton and
               Oriol Vinyals and
               Jeffrey Dean},
  title     = {Distilling the Knowledge in a Neural Network},
  journal   = {CoRR},
  volume    = {abs/1503.02531},
  year      = {2015},
  url       = {http://arxiv.org/abs/1503.02531},
  archivePrefix = {arXiv},
  eprint    = {1503.02531},
  timestamp = {Mon, 13 Aug 2018 16:48:36 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/HintonVD15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/iclr/MicikeviciusNAD18,
  author    = {Paulius Micikevicius and
               Sharan Narang and
               Jonah Alben and
               Gregory F. Diamos and
               Erich Elsen and
               David Garc{\'{\i}}a and
               Boris Ginsburg and
               Michael Houston and
               Oleksii Kuchaiev and
               Ganesh Venkatesh and
               Hao Wu},
  title     = {Mixed Precision Training},
  booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
               Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
  publisher = {OpenReview.net},
  year      = {2018},
  url       = {https://openreview.net/forum?id=r1gs9JgRZ},
  timestamp = {Thu, 25 Jul 2019 14:26:02 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/MicikeviciusNAD18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/aaai/DabreF19,
  author    = {Raj Dabre and
               Atsushi Fujita},
  title     = {Recurrent Stacking of Layers for Compact Neural Machine Translation
               Models},
  booktitle = {The Thirty-Third {AAAI} Conference on Artificial Intelligence, {AAAI}
               2019, The Thirty-First Innovative Applications of Artificial Intelligence
               Conference, {IAAI} 2019, The Ninth {AAAI} Symposium on Educational
               Advances in Artificial Intelligence, {EAAI} 2019, Honolulu, Hawaii,
               USA, January 27 - February 1, 2019},
  pages     = {6292--6299},
  publisher = {{AAAI} Press},
  year      = {2019},
  url       = {https://doi.org/10.1609/aaai.v33i01.33016292},
  doi       = {10.1609/aaai.v33i01.33016292},
  timestamp = {Wed, 25 Sep 2019 11:05:09 +0200},
  biburl    = {https://dblp.org/rec/conf/aaai/DabreF19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/emnlp/KimR16,
  author    = {Yoon Kim and
               Alexander M. Rush},
  editor    = {Jian Su and
               Xavier Carreras and
               Kevin Duh},
  title     = {Sequence-Level Knowledge Distillation},
  booktitle = {Proceedings of the 2016 Conference on Empirical Methods in Natural
               Language Processing, {EMNLP} 2016, Austin, Texas, USA, November 1-4,
               2016},
  pages     = {1317--1327},
  publisher = {The Association for Computational Linguistics},
  year      = {2016},
  url       = {https://doi.org/10.18653/v1/d16-1139},
  doi       = {10.18653/v1/d16-1139},
  timestamp = {Tue, 28 Jan 2020 10:28:22 +0100},
  biburl    = {https://dblp.org/rec/conf/emnlp/KimR16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/emnlp/ZophYMK16,
  author    = {Barret Zoph and
               Deniz Yuret and
               Jonathan May and
               Kevin Knight},
  editor    = {Jian Su and
               Xavier Carreras and
               Kevin Duh},
  title     = {Transfer Learning for Low-Resource Neural Machine Translation},
  booktitle = {Proceedings of the 2016 Conference on Empirical Methods in Natural
               Language Processing, {EMNLP} 2016, Austin, Texas, USA, November 1-4,
               2016},
  pages     = {1568--1575},
  publisher = {The Association for Computational Linguistics},
  year      = {2016},
  url       = {https://doi.org/10.18653/v1/d16-1163},
  doi       = {10.18653/v1/d16-1163},
  timestamp = {Tue, 28 Jan 2020 10:28:48 +0100},
  biburl    = {https://dblp.org/rec/conf/emnlp/ZophYMK16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/emnlp/NeubigH18,
  author    = {Graham Neubig and
               Junjie Hu},
  editor    = {Ellen Riloff and
               David Chiang and
               Julia Hockenmaier and
               Jun'ichi Tsujii},
  title     = {Rapid Adaptation of Neural Machine Translation to New Languages},
  booktitle = {Proceedings of the 2018 Conference on Empirical Methods in Natural
               Language Processing, Brussels, Belgium, October 31 - November 4, 2018},
  pages     = {875--880},
  publisher = {Association for Computational Linguistics},
  year      = {2018},
  url       = {https://doi.org/10.18653/v1/d18-1103},
  doi       = {10.18653/v1/d18-1103},
  timestamp = {Tue, 28 Jan 2020 10:28:36 +0100},
  biburl    = {https://dblp.org/rec/conf/emnlp/NeubigH18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/acl/SennrichHB16,
  author    = {Rico Sennrich and
               Barry Haddow and
               Alexandra Birch},
  title     = {Improving Neural Machine Translation Models with Monolingual Data},
  booktitle = {Proceedings of the 54th Annual Meeting of the Association for Computational
               Linguistics, {ACL} 2016, August 7-12, 2016, Berlin, Germany, Volume
               1: Long Papers},
  publisher = {The Association for Computer Linguistics},
  year      = {2016},
  url       = {https://doi.org/10.18653/v1/p16-1009},
  doi       = {10.18653/v1/p16-1009},
  timestamp = {Tue, 28 Jan 2020 10:28:01 +0100},
  biburl    = {https://dblp.org/rec/conf/acl/SennrichHB16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/emnlp/ZhangZ16,
  author    = {Jiajun Zhang and
               Chengqing Zong},
  editor    = {Jian Su and
               Xavier Carreras and
               Kevin Duh},
  title     = {Exploiting Source-side Monolingual Data in Neural Machine Translation},
  booktitle = {Proceedings of the 2016 Conference on Empirical Methods in Natural
               Language Processing, {EMNLP} 2016, Austin, Texas, USA, November 1-4,
               2016},
  pages     = {1535--1545},
  publisher = {The Association for Computational Linguistics},
  year      = {2016},
  url       = {https://doi.org/10.18653/v1/d16-1160},
  doi       = {10.18653/v1/d16-1160},
  timestamp = {Tue, 28 Jan 2020 10:28:36 +0100},
  biburl    = {https://dblp.org/rec/conf/emnlp/ZhangZ16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/acl/CollinsKK05,
  author    = {Michael Collins and
               Philipp Koehn and
               Ivona Kucerova},
  editor    = {Kevin Knight and
               Hwee Tou Ng and
               Kemal Oflazer},
  title     = {Clause Restructuring for Statistical Machine Translation},
  booktitle = {{ACL} 2005, 43rd Annual Meeting of the Association for Computational
               Linguistics, Proceedings of the Conference, 25-30 June 2005, University
               of Michigan, {USA}},
  pages     = {531--540},
  publisher = {The Association for Computer Linguistics},
  year      = {2005},
  url       = {https://www.aclweb.org/anthology/P05-1066/},
  doi       = {10.3115/1219840.1219906},
  timestamp = {Mon, 18 May 2020 15:12:39 +0200},
  biburl    = {https://dblp.org/rec/conf/acl/CollinsKK05.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/naacl/AharoniJF19,
  author    = {Roee Aharoni and
               Melvin Johnson and
               Orhan Firat},
  editor    = {Jill Burstein and
               Christy Doran and
               Thamar Solorio},
  title     = {Massively Multilingual Neural Machine Translation},
  booktitle = {Proceedings of the 2019 Conference of the North American Chapter of
               the Association for Computational Linguistics: Human Language Technologies,
               {NAACL-HLT} 2019, Minneapolis, MN, USA, June 2-7, 2019, Volume 1 (Long
               and Short Papers)},
  pages     = {3874--3884},
  publisher = {Association for Computational Linguistics},
  year      = {2019},
  url       = {https://doi.org/10.18653/v1/n19-1388},
  doi       = {10.18653/v1/n19-1388},
  timestamp = {Tue, 28 Jan 2020 10:30:14 +0100},
  biburl    = {https://dblp.org/rec/conf/naacl/AharoniJF19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/coling/BlackwoodBW18,
  author    = {Graeme W. Blackwood and
               Miguel Ballesteros and
               Todd Ward},
  editor    = {Emily M. Bender and
               Leon Derczynski and
               Pierre Isabelle},
  title     = {Multilingual Neural Machine Translation with Task-Specific Attention},
  booktitle = {Proceedings of the 27th International Conference on Computational
               Linguistics, {COLING} 2018, Santa Fe, New Mexico, USA, August 20-26,
               2018},
  pages     = {3112--3122},
  publisher = {Association for Computational Linguistics},
  year      = {2018},
  url       = {https://www.aclweb.org/anthology/C18-1263/},
  timestamp = {Mon, 16 Sep 2019 17:08:53 +0200},
  biburl    = {https://dblp.org/rec/conf/coling/BlackwoodBW18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/wmt/SachanN18,
  author    = {Devendra Singh Sachan and
               Graham Neubig},
  editor    = {Ondrej Bojar and
               Rajen Chatterjee and
               Christian Federmann and
               Mark Fishel and
               Yvette Graham and
               Barry Haddow and
               Matthias Huck and
               Antonio Jimeno{-}Yepes and
               Philipp Koehn and
               Christof Monz and
               Matteo Negri and
               Aur{\'{e}}lie N{\'{e}}v{\'{e}}ol and
               Mariana L. Neves and
               Matt Post and
               Lucia Specia and
               Marco Turchi and
               Karin Verspoor},
  title     = {Parameter Sharing Methods for Multilingual Self-Attentional Translation
               Models},
  booktitle = {Proceedings of the Third Conference on Machine Translation: Research
               Papers, {WMT} 2018, Belgium, Brussels, October 31 - November 1, 2018},
  pages     = {261--271},
  publisher = {Association for Computational Linguistics},
  year      = {2018},
  url       = {https://doi.org/10.18653/v1/w18-6327},
  doi       = {10.18653/v1/w18-6327},
  timestamp = {Tue, 28 Jan 2020 10:30:59 +0100},
  biburl    = {https://dblp.org/rec/conf/wmt/SachanN18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/rep4nlp/VazquezRTC19,
  author    = {Ra{\'{u}}l V{\'{a}}zquez and
               Alessandro Raganato and
               J{\"{o}}rg Tiedemann and
               Mathias Creutz},
  editor    = {Isabelle Augenstein and
               Spandana Gella and
               Sebastian Ruder and
               Katharina Kann and
               Burcu Can and
               Johannes Welbl and
               Alexis Conneau and
               Xiang Ren and
               Marek Rei},
  title     = {Multilingual {NMT} with a Language-Independent Attention Bridge},
  booktitle = {Proceedings of the 4th Workshop on Representation Learning for NLP,
               RepL4NLP@ACL 2019, Florence, Italy, August 2, 2019},
  pages     = {33--39},
  publisher = {Association for Computational Linguistics},
  year      = {2019},
  url       = {https://doi.org/10.18653/v1/w19-4305},
  doi       = {10.18653/v1/w19-4305},
  timestamp = {Fri, 27 Mar 2020 08:52:29 +0100},
  biburl    = {https://dblp.org/rec/conf/rep4nlp/VazquezRTC19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-2004-06575,
  author    = {Carlos Escolano and
               Marta R. Costa{-}juss{\`{a}} and
               Jos{\'{e}} A. R. Fonollosa and
               Mikel Artetxe},
  title     = {Multilingual Machine Translation: Closing the Gap between Shared and
               Language-specific Encoder-Decoders},
  journal   = {CoRR},
  volume    = {abs/2004.06575},
  year      = {2020},
  url       = {https://arxiv.org/abs/2004.06575},
  archivePrefix = {arXiv},
  eprint    = {2004.06575},
  timestamp = {Tue, 21 Apr 2020 16:51:52 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2004-06575.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/emnlp/BapnaF19,
  author    = {Ankur Bapna and
               Orhan Firat},
  editor    = {Kentaro Inui and
               Jing Jiang and
               Vincent Ng and
               Xiaojun Wan},
  title     = {Simple, Scalable Adaptation for Neural Machine Translation},
  booktitle = {Proceedings of the 2019 Conference on Empirical Methods in Natural
               Language Processing and the 9th International Joint Conference on
               Natural Language Processing, {EMNLP-IJCNLP} 2019, Hong Kong, China,
               November 3-7, 2019},
  pages     = {1538--1548},
  publisher = {Association for Computational Linguistics},
  year      = {2019},
  url       = {https://doi.org/10.18653/v1/D19-1165},
  doi       = {10.18653/v1/D19-1165},
  timestamp = {Thu, 12 Dec 2019 13:23:44 +0100},
  biburl    = {https://dblp.org/rec/conf/emnlp/BapnaF19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/iclr/BauBSDDG19,
  author    = {Anthony Bau and
               Yonatan Belinkov and
               Hassan Sajjad and
               Nadir Durrani and
               Fahim Dalvi and
               James R. Glass},
  title     = {Identifying and Controlling Important Neurons in Neural Machine Translation},
  booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
               New Orleans, LA, USA, May 6-9, 2019},
  publisher = {OpenReview.net},
  year      = {2019},
  url       = {https://openreview.net/forum?id=H1z-PsR5KX},
  timestamp = {Thu, 25 Jul 2019 14:25:45 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/BauBSDDG19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/acl/VoitaTMST19,
  author    = {Elena Voita and
               David Talbot and
               Fedor Moiseev and
               Rico Sennrich and
               Ivan Titov},
  editor    = {Anna Korhonen and
               David R. Traum and
               Llu{\'{\i}}s M{\`{a}}rquez},
  title     = {Analyzing Multi-Head Self-Attention: Specialized Heads Do the Heavy
               Lifting, the Rest Can Be Pruned},
  booktitle = {Proceedings of the 57th Conference of the Association for Computational
               Linguistics, {ACL} 2019, Florence, Italy, July 28- August 2, 2019,
               Volume 1: Long Papers},
  pages     = {5797--5808},
  publisher = {Association for Computational Linguistics},
  year      = {2019},
  url       = {https://doi.org/10.18653/v1/p19-1580},
  doi       = {10.18653/v1/p19-1580},
  timestamp = {Tue, 28 Jan 2020 10:27:29 +0100},
  biburl    = {https://dblp.org/rec/conf/acl/VoitaTMST19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/iclr/MolchanovTKAK17,
  author    = {Pavlo Molchanov and
               Stephen Tyree and
               Tero Karras and
               Timo Aila and
               Jan Kautz},
  title     = {Pruning Convolutional Neural Networks for Resource Efficient Inference},
  booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
               Toulon, France, April 24-26, 2017, Conference Track Proceedings},
  publisher = {OpenReview.net},
  year      = {2017},
  url       = {https://openreview.net/forum?id=SJGCiw5gl},
  timestamp = {Thu, 25 Jul 2019 14:25:44 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/MolchanovTKAK17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:journals/jmlr/GlorotBB11,
  author    = {Xavier Glorot and
               Antoine Bordes and
               Yoshua Bengio},
  editor    = {Geoffrey J. Gordon and
               David B. Dunson and
               Miroslav Dud{\'{\i}}k},
  title     = {Deep Sparse Rectifier Neural Networks},
  booktitle = {Proceedings of the Fourteenth International Conference on Artificial
               Intelligence and Statistics, {AISTATS} 2011, Fort Lauderdale, USA,
               April 11-13, 2011},
  series    = {{JMLR} Proceedings},
  volume    = {15},
  pages     = {315--323},
  publisher = {JMLR.org},
  year      = {2011},
  url       = {http://proceedings.mlr.press/v15/glorot11a/glorot11a.pdf},
  timestamp = {Wed, 29 May 2019 08:41:47 +0200},
  biburl    = {https://dblp.org/rec/journals/jmlr/GlorotBB11.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/conll/SeeLM16,
  author    = {Abigail See and
               Minh{-}Thang Luong and
               Christopher D. Manning},
  editor    = {Yoav Goldberg and
               Stefan Riezler},
  title     = {Compression of Neural Machine Translation Models via Pruning},
  booktitle = {Proceedings of the 20th {SIGNLL} Conference on Computational Natural
               Language Learning, CoNLL 2016, Berlin, Germany, August 11-12, 2016},
  pages     = {291--301},
  publisher = {{ACL}},
  year      = {2016},
  url       = {https://doi.org/10.18653/v1/k16-1029},
  doi       = {10.18653/v1/k16-1029},
  timestamp = {Tue, 28 Jan 2020 10:29:27 +0100},
  biburl    = {https://dblp.org/rec/conf/conll/SeeLM16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{post-2018-call,
  title = "A Call for Clarity in Reporting {BLEU} Scores",
  author = "Post, Matt",
  booktitle = "Proceedings of the Third Conference on Machine Translation: Research Papers",
  month = oct,
  year = "2018",
  address = "Belgium, Brussels",
  publisher = "Association for Computational Linguistics",
  url = "https://www.aclweb.org/anthology/W18-6319",
  pages = "186--191",
}

@inproceedings{
zhang2021share,
title={Share or Not? Learning to Schedule Language-Specific Capacity for Multilingual Translation},
author={Biao Zhang and Ankur Bapna and Rico Sennrich and Orhan Firat},
booktitle={International Conference on Learning Representations},
year={2021},
url={https://openreview.net/forum?id=Wj4ODo0uyCF}
}

@inproceedings{DBLP:conf/iclr/ZhuG18,
  author    = {Michael Zhu and
               Suyog Gupta},
  title     = {To Prune, or Not to Prune: Exploring the Efficacy of Pruning for Model
               Compression},
  booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
               Vancouver, BC, Canada, April 30 - May 3, 2018, Workshop Track Proceedings},
  publisher = {OpenReview.net},
  year      = {2018},
  url       = {https://openreview.net/forum?id=Sy1iIDkPM},
  timestamp = {Thu, 04 Apr 2019 13:20:09 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/ZhuG18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/emnlp/WangWLT20,
  author    = {Yong Wang and
               Longyue Wang and
               Victor O. K. Li and
               Zhaopeng Tu},
  editor    = {Bonnie Webber and
               Trevor Cohn and
               Yulan He and
               Yang Liu},
  title     = {On the Sparsity of Neural Machine Translation Models},
  booktitle = {Proceedings of the 2020 Conference on Empirical Methods in Natural
               Language Processing, {EMNLP} 2020, Online, November 16-20, 2020},
  pages     = {1060--1066},
  publisher = {Association for Computational Linguistics},
  year      = {2020},
  url       = {https://doi.org/10.18653/v1/2020.emnlp-main.78},
  doi       = {10.18653/v1/2020.emnlp-main.78},
  timestamp = {Fri, 08 Jan 2021 21:21:09 +0100},
  biburl    = {https://dblp.org/rec/conf/emnlp/WangWLT20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/iclr/LanCGGSS20,
  author    = {Zhenzhong Lan and
               Mingda Chen and
               Sebastian Goodman and
               Kevin Gimpel and
               Piyush Sharma and
               Radu Soricut},
  title     = {{ALBERT:} {A} Lite {BERT} for Self-supervised Learning of Language
               Representations},
  booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
               Addis Ababa, Ethiopia, April 26-30, 2020},
  publisher = {OpenReview.net},
  year      = {2020},
  url       = {https://openreview.net/forum?id=H1eA7AEtvS},
  timestamp = {Thu, 07 May 2020 17:11:48 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/LanCGGSS20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/iccv/LuoWL17,
  author    = {Jian{-}Hao Luo and
               Jianxin Wu and
               Weiyao Lin},
  title     = {ThiNet: {A} Filter Level Pruning Method for Deep Neural Network Compression},
  booktitle = {{IEEE} International Conference on Computer Vision, {ICCV} 2017, Venice,
               Italy, October 22-29, 2017},
  pages     = {5068--5076},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/ICCV.2017.541},
  doi       = {10.1109/ICCV.2017.541},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/iccv/LuoWL17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/aaai/WangWSLT20,
  author    = {Yong Wang and
               Longyue Wang and
               Shuming Shi and
               Victor O. K. Li and
               Zhaopeng Tu},
  title     = {Go From the General to the Particular: Multi-Domain Translation with
               Domain Transformation Networks},
  booktitle = {The Thirty-Fourth {AAAI} Conference on Artificial Intelligence, {AAAI}
               2020, The Thirty-Second Innovative Applications of Artificial Intelligence
               Conference, {IAAI} 2020, The Tenth {AAAI} Symposium on Educational
               Advances in Artificial Intelligence, {EAAI} 2020, New York, NY, USA,
               February 7-12, 2020},
  pages     = {9233--9241},
  publisher = {{AAAI} Press},
  year      = {2020},
  url       = {https://aaai.org/ojs/index.php/AAAI/article/view/6461},
  timestamp = {Fri, 03 Jul 2020 17:58:11 +0200},
  biburl    = {https://dblp.org/rec/conf/aaai/WangWSLT20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
